Ruling polynomials and augmentations over finite fields

For any Legendrian link, L, in (\R^3, \ker(dz-y\,dx)) we define invariants, Aug_m(L,q), as normalized counts of augmentations from the Legendrian contact homology DGA of L into a finite field of order q where the parameter m is a divisor of twice the rotation number of L. Generalizing a result of Ng and Sabloff for the case q =2, we show the augmentation numbers, Aug_m(L,q), are determined by specializing the m-graded ruling polynomial, R^m_L(z), at z = q^{1/2}-q^{-1/2}. As a corollary, we deduce that the ruling polynomials are determined by the Legendrian contact homology DGA.

==> Sections/Preamble.tex <==
% This is the preamble of the document where Theorem-type environments are defined. Common shortcuts and document-specific notation are also defined here.
% Michael Brad Henry

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\makeatletter
\newtheorem*{rep@corollary}{\rep@title}
\newcommand{\newrepcorollary}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@corollary}}%
 {\end{rep@corollary}}}
\makeatother

% Theorems and such
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newreptheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newrepcorollary{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{property}{Property}
\newtheorem{step}{Step}
\newtheorem*{condition}{Condition}
\newtheorem{question}{Question}
\newtheorem{remark}[theorem]{Remark}

\theoremstyle{remark}
\newtheorem*{example}{Example}
\newtheorem*{note}{Note}


% Shortcut to ``blackboard bold'' and script letters
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\pp}{\ensuremath{\mathbb{P}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\aac}{\ensuremath{\mathcal{A}}}
\newcommand{\bbc}{\ensuremath{\mathcal{B}}}
\newcommand{\rrc}{\ensuremath{\mathcal{R}}}
\newcommand{\wwc}{\ensuremath{\mathcal{W}}}
\newcommand{\vvc}{\ensuremath{\mathcal{V}}}
\newcommand{\ttc}{\ensuremath{\mathcal{T}}}
\newcommand{\ssc}{\ensuremath{\mathcal{S}}}
\newcommand{\llc}{\ensuremath{\mathcal{L}}}
\newcommand{\kkc}{\ensuremath{\mathcal{K}}}
\newcommand{\nnc}{\ensuremath{\mathcal{N}}}
\newcommand{\xxc}{\ensuremath{\mathcal{X}}}
\newcommand{\mmc}{\ensuremath{\mathcal{M}}}

\newcommand{\cc}{\ensuremath{\mathbb{C}}}

\newcommand{\aug}{\ensuremath{\epsilon}}
\newcommand{\MCS}{\ensuremath{\mathcal{C}}}
\newcommand{\Leg}{\ensuremath{L}}
\newcommand{\ruling}{\ensuremath{\rho}}
\newcommand{\front}{\ensuremath{D}}
\newcommand{\ring}{\ensuremath{R}}
\newcommand{\field}{\ensuremath{\mathbb{F}}}
\newcommand{\Maslov}{\ensuremath{\mu}}
\newcommand{\Zm}{\ensuremath{\mathbb{Z} / m \mathbb{Z}}}

%Brad:  Some of thesee notations may look nicer if you use $\mathit{Aug}_m(D;\F)$ which will typeset slightly differently than $Aug_m(D;\F)$.  In the latter the Aug part is designed to appear as a product of A u and g.

%Notation agreed upon during Dan's visit to Siena
%
%Legendrian knot/link: $L$
%
%Normal ruling: $\rho$
%
%Grading: $m$
%
%Field: $\mathbb{F}$ (or shortcut $\F$)
%
%A prime number: $p$ 
%
%Front diagram of $L$: $D$
%
%CE-DGA of $D$: $(\mathcal{A}(D), \partial)$
%
%The set of $m$-graded augmentations to $F$ of $(\mathcal{A}(D), \partial)$:  $\overline{Aug}_m(D;\F)$
%
%Normalized $m$-graded augmentation invariant: $Aug_m(D;\F)$
%
%The set of $A$-form $m$-graded MCSs over $\F$: $MCS_m^{A}(D;\F)$
%
%The set of $SR$-form $m$-graded MCSs over $\F$: $MCS_m^{SR}(D;\F)$


%Extra and possibly unnecessary code of unknown origin. I am hesistant to remove it until I am sure it is unneeded.

% Adrian's magic label command
\newcommand{\mylabel}[1]{\label{#1}
%Comment this part out to remove the label boxes
%\fbox{\upshape \tiny {#1}}
}

\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
}
\providecommand{\href}[2]{#2}
